AST-Based Automated Elimination of break and continue Statements in Java Code

This work presents the development of an automatic refactoring tool for Java code built on top of the Eclipse JDT API. The proposed approach transforms control structures containing break and continue statements within different types of loops into semantically equivalent constructs that avoid their explicit use. To achieve this, auxiliary boolean variables are introduced to restructure the control flow while preserving the original program behavior. The main objective of this transformation is to improve code structure and enable the application of subsequent automated refactorings, particularly those based on the Extract Method operation, which are typically restricted by the presence of jump statements. The implementation relies on the analysis and rewriting of the Abstract Syntax Tree (AST), ensuring semantic equivalence in all addressed scenarios. The tool was validated through 54 manually designed test cases and 151 units tests, all of which produced satisfactory results. In addition, it was applied to 139 methods from seven open-source projects, generating code without compilation errors and preserving the original behavior as verified by the projects' test suites. The results demonstrate that the proposed approach safely automates the restructuring of code containing break and continue statements, facilitating further evolution and structural analysis.

==> datos.tex <==
\def \alumno {Nombre de alumno}
\def \tutor {Nombre del tutor}
\def \cotutor {Nombre del cotutor} % optional (comment if none)
\def \departamento {Nombre del departamento}
\def \grado {Nombre del grado}
\def \facultad {Nombre de la facultad}
\def \fecha {Fecha}
\def \tituloes {Título en ES}
\def \tituloen {Título en EN}
\def \subtituloes {Subtítulo en ES} % optional (comment if none)
\def \subtituloen {Subtítulo en EN} % optional (comment if none)

% Extra pages
\def \addacknowledgments {} % optional: comment this line if you don't want to include acknowledgments
\def \addappendix {}  % optional: comment this line if you don't want to include appendix
\def \configpar {} % optional: comment this line if you don't want first-line indents in paragraphs


==> pages/02-portada.tex <==
\begin{center}
  \begin{figure*}[h]
    \centering
    \includegraphics[scale=0.2]{images/00-marcauma.png}
  \end{figure*}

  \MakeUppercase{\facultad} \\
  GRADO EN \MakeUppercase{\grado} \\
  \vspace{3cm}
  {\large	\tituloes} \\
  \ifdef{\subtituloes}{
    \textit{\subtituloes} \\
  }{}
  {\large	\tituloen} \\
  \ifdef{\subtituloen}{
    \textit{\subtituloen} \\
  }{}  \bigbreak
  Realizado por \\
  \textbf{\alumno} \\
  Tutorizado por \\
  \textbf{\tutor} \\
  \ifdef{\cotutor}{
    Cotutorizado por \\
    \textbf{\cotutor} \\
  }{}
  Departamento \\
  \textbf{\departamento}
  \bigbreak
  UNIVERSIDAD DE MÁLAGA \\
  MÁLAGA, \fecha
\end{center}

\vfill

Fecha defensa: \\
El Secretario del Tribunal


==> pages/04-resumen.tex <==
This work presents the development of an automatic refactoring tool for Java code built on top of the Eclipse JDT API. The proposed approach transforms control structures containing \texttt{break} and \texttt{continue} statements within different types of loops into semantically equivalent constructs that avoid their explicit use. To achieve this, auxiliary boolean variables are introduced to restructure the control flow while preserving the original program behavior.

The main objective of this transformation is to improve code structure and enable the application of subsequent automated refactorings, particularly those based on the Extract Method operation, which are typically restricted by the presence of jump statements. The implementation relies on the analysis and rewriting of the Abstract Syntax Tree (AST), ensuring semantic equivalence in all addressed scenarios.

The tool was validated through 54 manually designed test cases and 151 units tests, all of which produced satisfactory results. In addition, it was applied to 139 methods from seven open-source projects, generating code without compilation errors and preserving the original behavior as verified by the projects’ test suites.

The results demonstrate that the proposed approach safely automates the restructuring of code containing break and continue statements, facilitating further evolution and structural analysis.


\textbf{Keywords}: Java, Eclipse JDT, Abstract Syntax Tree, Code Refactoring, Method Extraction, Control Flow Transformation, \texttt{break}, \texttt{continue}, Static Analysis.



==> pages/06-anexos.tex <==
%\chapter{Ejemplo de anexo}
%\label{appendix:examples}

\appendix
\chapter{Repository and Source Code}
\label{anexo:repositorio}

To facilitate the reproducibility of the results and the reuse of the tool, the complete source code has been published in a public GitHub repository.

\section{Structure of the Repository}
The repository is organized into the following directories:

\begin{itemize}
    \item \texttt{org.plugin.refactor.code}: Implementation of the automated refactoring tool developed using the Eclipse JDT API (plugin).
    \item \texttt{refactoring-core-clean}: A Maven project containing the suite of 151 tests used during validation, including cases with \texttt{while}, \texttt{for}, \texttt{do-while}, and \texttt{enhanced-for} loops, as well as structures with exception handling.
    \item \texttt{evaluation-projects}: A set of external projects used to evaluate the tool in real-world scenarios. This directory contains two subdirectories:
    \begin{itemize}
        \item \texttt{original}: The original versions of the projects used as input for the tool.
        \item \texttt{refactored}: The versions resulting from the automated refactoring process.
    \end{itemize}
\end{itemize}

\section{Access and Cloning}
The code is available at the following URL: \\
\url{https://github.com/andyjuarez-dev/automated-refactoring-java-code.git}

To clone the repository, use the following command:
\begin{center}
    \texttt{git clone https://github.com/andyjuarez-dev/automated-refactoring-java-code.git}
\end{center}

It is highly recommended to consult the \texttt{README.md} file included in the repository, which provides detailed instructions for the configuration and execution of the tool.


\chapter{Refactored Method Examples}
\label{anexo:ejemplos-codigo}

This appendix presents representative case studies that illustrate the transformation capabilities of the developed plugin. The selected methods comprise both controlled laboratory scenarios specifically designed to examine particular aspects of the transformation process and real-world examples from open-source projects analyzed during the experiments. Together, they provide a comparative view of the original code versus the refactored version.

\section{Controlled Laboratory Scenarios}
The following sections document the controlled laboratory scenarios developed for this research. These synthetic benchmarks were designed to validate the correctness of the refactoring algorithms under stable and reproducible conditions. Each scenario focuses on a specific architectural challenge, providing the necessary context for the results discussed in Chapter 6.

\subsection{Case 7: \texttt{while-breaks-continues}}
\label{subsec:B-case7-while-breaks-continues}

The instance presented below demonstrates a complex control flow: a \texttt{while} loop containing a \texttt{continue} statement is situated inside a \texttt{do-while} loop, which also incorporates a \texttt{break} statement at the third level of nesting. Notably, both control transfer statements are followed by subsequent executable code.

\begin{listing}[ht]
	\caption{Case 7: \texttt{while} and \texttt{do-while} loops. Original code.}
	\label{lst:B-case7-original}
	\begin{minipage}{\linewidth}
	\begin{minted}[highlightlines={13, 19, 23}]{java}
public void m() {
	int z = 6;
	System.out.println(z);
	int x = 5;
	int cond = 3;
	do {
		int y = 10;
		double w;
		if (x == 5) {
			if (z % 2 == 0) {
				if (cond == 3) {
					System.out.println(cond);
					break;
				}
				w = 3.14;
			}
			x++;
		} else
			continue;
		while (y < 10) {
			y++;
			if (y == 8)
				continue;
			System.out.println("valor de y: " + y);
		}
		z++;
		y++;
	} while (x < 10);
}
	\end{minted}
	\end{minipage}
\end{listing}


\begin{listing}[ht]
	\caption{Refactoring of Listing \ref{lst:B-case7-original}.}
	\label{lst:B-case7-refactored}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={6,8,15,17,19,21,23,25,26,28,31,32,34,39}]{java}
public void m() {
	int z = 6;
	System.out.println(z);
	int x = 5;
	int cond = 3;
	boolean stay1 = true;
	do {
		boolean keep1 = true;
		int y = 10;
		double w;
		if (x == 5) {
			if (z % 2 == 0) {
				if (cond == 3) {
					System.out.println(cond);
					stay1 = false;
				}
				if (stay1) { 
					w = 3.14; 
				}
			}
			if (stay1) { 
				x++; 
			}
		} else
		keep1 = false;
		if (stay1 && keep1) {
			while (y < 10) {
				boolean keep2 = true;
				y++;
				if (y == 8)
					keep2 = false;
				if (keep2) {
					System.out.println("valor de y: " + y);
				}
			}
			z++;
			y++;
		}
	} while (stay1 && (x < 10));
}
	\end{minted}
	\end{minipage}
\end{listing}

	
\subsection{Case 9: \texttt{for-breaks-continues}}
\label{subsec:B-case9-for-breaks-continues}

The following case illustrates the refactoring of a \texttt{for} loop characterized by nested \texttt{break} and \texttt{continue} instructions. Note that the original structure is replaced by a \texttt{while} loop to maintain semantic equivalence throughout the transformation.

\begin{listing}[ht]
	\caption{Case 9: \texttt{for} loop. Original code.}
	\label{lst:B-case9-original}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={7,11}]{java}
public void m() {
	int x = 0;
	for (int i = 0; i < 10; i++) {
		System.out.println("Hello");
		if (i == 5)
			if (x % 2 == 0)
				break;
		x++;
		if (x < 10) {
			continue;
		}
		x *= 2;
		System.out.println("End for");
	}
	System.out.println("End m");
}		
	\end{minted}
	\end{minipage}
\end{listing}

\begin{listing}[ht]
	\caption{Refactoring of Listing \ref{lst:B-case9-original}.}
	\label{lst:B-case9-refactored}
	\begin{minipage}{\linewidth}
	\begin{minted}[highlightlines={3,4,5,6,7,8,12,13,16,18,21,22,23,24,26,28}]{java}
public void m() {
	int x = 0;
	{
		int i = 0;
		boolean stay1 = true;
		while (stay1 && (i < 10)) {
			boolean keep1 = true;
			{
				System.out.println("Hello");
				if (i == 5)
					if (x % 2 == 0)
						stay1 = false;
				if (stay1) {
					x++;
					if (x < 10) {
						keep1 = false;
					}
					if (keep1) {
						x *= 2;
						System.out.println("End for");
					}
				}
			}
			if (stay1) {
				i++;
			}
		}
	}
	System.out.println("End m");
}
	\end{minted}
	\end{minipage}
\end{listing}


\subsection{Case 10: \texttt{foreach-breaks-continues}}
\label{subsec:B-case10-foreach-breaks-continues}

This scenario is analogous to Case 9, but utilizes a \texttt{for-each} loop as the primary iteration structure. The key distinction in this transformation lies in the underlying data structures handled by the application, as well as the inclusion of specific libraries required for iterator management.

\begin{listing}[ht]
	\caption{Case 10: \texttt{foreach} loop. Original code}
	\label{lst:B-case10-original}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={17,24}]{java}
import java.util.ArrayList;
import java.util.List;
			
public class Example {
	public void m() {
		int x = 0;
		String vec[] = {"Peter", "John", "Mary"};
		List<String> ls = new ArrayList<>();
					
		ls.add("Peter"); 
		ls.add("John");
		ls.add("Mary");
					
		for(String s: ls) {
			System.out.println("Name: " + s);
			if (s.equals("John"))
				break;
			x++;
		}
					
		for(String s: vec) {
			System.out.println("Name: " + s);
			if (s.equals("John"))
				break;
			x++;
		}
	}
}
		\end{minted}
	\end{minipage}
\end{listing}


\begin{listing}[ht]
	\caption{Refactored version of the \texttt{foreach} loops.}
	\label{lst:B-case10-refactored}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={3,4,13,14,15,16,19,20,22,25,26,27,28,31,32,34}]{java}
import java.util.ArrayList;
import java.util.List;
import java.util.Iterator;
import java.util.Arrays;
			
public class Example {
	public void m() {
		int x = 0;
		String vec[] = {"Peter", "John", "Mary"};
		List<String> ls = new ArrayList<>();
		// ... list population ...
					
		Iterator<String> it = ls.iterator();
		boolean stay1 = true;
		while (stay1 && (it.hasNext())) {
			String s = it.next();
			System.out.println("Name: " + s);
			if (s.equals("John"))
			stay1 = false;
			if (stay1) { 
				x++; 
			}
		}
					
		Iterator<String> it1 = Arrays.stream(vec).iterator();
		boolean stay2 = true;
		while (stay2 && (it1.hasNext())) {
			String s = it1.next();
			System.out.println("Name: " + s);
			if (s.equals("John"))
			stay2 = false;
			if (stay2) { 
				x++; 
			}
		}
	}
}
		\end{minted}
	\end{minipage}
\end{listing}



%
%% Configuración de listings para Java
%\lstset{
%    language=Java,
%    basicstyle=\ttfamily\small,
%    keywordstyle=\color{blue}\bfseries,
%    commentstyle=\color{gray},
%    stringstyle=\color{red},
%    numbers=left,
%    numberstyle=\tiny\color{gray},
%    stepnumber=1,
%    numbersep=10pt,
%    backgroundcolor=\color{white},
%    showspaces=false,
%    showstringspaces=false,
%    showtabs=false,
%    frame=single,
%    tabsize=2,
%    captionpos=b,
%    breaklines=true,
%    breakatwhitespace=true,
%}
%

\subsection{Case 13: Nested Exceptions}
\label{subsec:B-nested-exceptions}

A complex scenario involving a \texttt{while} loop with nested exceptions and multiple \texttt{break} statements. This case evaluates the algorithm's robustness when dealing with intricate control flows, where exception-handling blocks and control transfer statements are deeply interleaved.

\begin{listing}[ht]
	\caption{Nested exceptions with \texttt{breaks}. Original code.}
	\label{lst:B-case13-nested-exceptions-original}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={7,10,13,16,21,24}]{java}
public void m() {
    int i = 0;
    while (i < 2) {
        i++;
        System.out.println("Statement 1");
        try {
            if (dev(2)) break;
            System.out.println("Statement 4");             
            try {
                if (dev(3)) break;
                System.out.println("Statement 6");                    
            } catch(Exception e) {
                if (dev(4)) break;
                System.out.println("Statement 8");
            } finally {
                if (dev(5)) break;
                System.out.println("Statement 10");                    
            }
            System.out.println("Statement 11");    
        } catch(Exception e) {
            if (dev(6)) break;
            System.out.println("Statement 13");
        } finally {
            if (dev(7)) break;
            System.out.println("Statement 15");                             
        }
        System.out.println("Statement 16");    
    }
}
	\end{minted}
	\end{minipage}
\end{listing}

%\newpage
%

\begin{listing}[ht]
	\caption{Refactored version of Listing \ref{lst:B-case13-nested-exceptions-original}.}
	\label{lst:B-refac-exceptions}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={3,4,5,6,10,11,14,15,17,19,20,22,24,25,27,29,31,32,34,35,37,39,40,42,44,46}]{java}
public void m() {
    int i = 0;
    boolean stay1 = true;
    boolean stay3 = true;
    boolean stay2 = true;
    while (stay1 && stay3 && stay2 && (i < 2)) {
        i++;
        System.out.println("Statement 1");
        try {
            if (dev(2)) stay1 = false;
            if (stay1) {
                System.out.println("Statement 4");
                try {
                    if (dev(3)) stay1 = false;
                    if (stay1) {
                        System.out.println("Statement 6");
                    }                                
                } catch(Exception e) {
                    if (dev(4)) stay1 = false;
                    if (stay1) {
                        System.out.println("Statement 8");
                    }
                } finally {
                    if (dev(5)) stay2 = false;
                    if (stay2) {
                        System.out.println("Statement 10");
                    }                                
                }
                if (stay1 && stay2) {
                    System.out.println("Statement 11");
                }
            }      
        } catch(Exception e) {
            if (dev(6)) stay1 = false;
            if (stay1) {
                System.out.println("Statement 13");
            }
        } finally {
            if (dev(7)) stay3 = false;
            if (stay3) {
                System.out.println("Statement 15");
            }                                
        }
        if (stay3 && stay1 && stay2) {
            System.out.println("Statement 16");
        }                          
    }
}
	\end{minted}
	\end{minipage}
\end{listing}

\FloatBarrier

\section{Real-world Projects}
\label{sec:real-world-projects}

From the 139 transformed methods, two were selected from the MOEAFramework project for detailed analysis: evaluate and calculateEfficiency. The rationale for selecting the former is based on the project’s test suite, which directly targeted this method and confirmed its successful execution. The latter was chosen because external tools failed to reduce its complexity below the threshold recommended by SonarSource. While Listing XX demonstrates a significant reduction in cognitive complexity through the manual application of the 'Extract Method' pattern, it remained above the target level of 15.

%% Seccion de proyectos reales (MOEAFramework)
%\section{Real-world Project Cases}
 %

\subsection{MOEAFramework Project}
\label{subsec:MOEAFramework}
 
\begin{listing}[ht]
	\caption{Method \texttt{evaluate} (MOEAFramework). Original code.}
	\label{lst:moea-orig}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={10,16}]{java}
public double evaluate(NondominatedPopulation approximationSet) {
    int count = 0;
    for (Solution solution1: referenceSet) {
        boolean match = false;
        for (Solution solution2: approximationSet) {
            if (comparator == null) {
                double distance = MathArrays.distance(solution1.getObjectives(), solution2.getObjectives());
                if (distance < Settings.EPS) {
                    match = true;
                    break;
                }
            } else {
                comparator.compare(solution1, solution2);
                if (comparator.isSameBox()) {
                    match = true;
                    break;
                }
            }
        }
        if (match) {
            count++;
        }
    }
    return count / (double)referenceSet.size();
}
	\end{minted}
	\end{minipage}
\end{listing}


\begin{listing}[ht]
	\caption{Method \texttt{evaluate} (MOEAFramework). Refactored code.}
	\label{lst:moea-refac}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={5,6,7,8,13,19}]{java}
public double evaluate(NondominatedPopulation approximationSet) {
    int count = 0;
    for (Solution solution1 : referenceSet) {
        boolean match = false;
        Iterator<Solution> it = approximationSet.iterator();
        boolean stay1 = true;
        while (stay1 && (it.hasNext())) {
            Solution solution2 = it.next();
            if (comparator == null) {
                double distance = MathArrays.distance(solution1.getObjectives(), solution2.getObjectives());
                if (distance < Settings.EPS) {
                    match = true;
                    stay1 = false;
                }
            } else {
                comparator.compare(solution1, solution2);
                if (comparator.isSameBox()) {
                    match = true;
                    stay1 = false;
                }
            }
        }
        if (match) {
            count++;
        }
    }
    return count / (double)referenceSet.size();
}
	\end{minted}
	\end{minipage}
\end{listing}



\subsection{Case Study: Manual Refinement of Complex Logic in calculateEfficiency}
\label{subsec:facilitating-extract-method}

While the automated refactoring tool successfully restructured the method, the resulting Cognitive Complexity (CC) remained at 24, exceeding the recommended threshold of 15. By manually applying the 'Extract Method' pattern to the most deeply nested structures, the complexity was further reduced to 17. Although this value remains slightly above the ideal limit, this 29\% reduction (from 24 to 17) demonstrates that manual refinement can significantly optimize results in some scenarios. 

\begin{listing}[ht]
	\caption{Method calculateEfficiency after internal refactoring.}
	\label{lst:calc-eff-internal}
	\begin{minipage}{\linewidth}
	\begin{minted}{java}
private double calculateEfficiency() {
	//find the max evaluations parameter index
	int max = -1;
	int evalIndex = -1;
	int i7 = 0;
	boolean stay1 = true;
	while (stay1 && (i7 < parameterFile.size())) {
		Parameter parameter = parameterFile.get(i7);
		if (parameter.getName().equals("maxEvaluations")) {
			max = (int) parameter.getUpperBound();
			evalIndex = i7;
			stay1 = false;
		}
		if (stay1) {
			i7++;
		}
	}
	if (evalIndex == -1) {
		throw new FrameworkException("no maxEvaluations parameter");
	}
	//find lowest band reaching attainment
	int band = max;
	int i8 = 0;
	boolean stay2 = true;
	while (stay2 && (i8 <= max - bandWidth)) {
		int count = 0;
		int total = 0;
		for (int j = 0; j < metrics.length; j++) {
			if ((parameters[j][evalIndex] >= i8) && 
             (parameters[j][evalIndex] <= i8 + bandWidth - 1)) {
				total++;
				if (metrics[j][metric] > threshold) {
					count++;
					if (count / (double) total >= 0.9) {
						band = i8;
						stay2 = false;
					}
				}
			}
		}
		i8 += bandWidth;
	}
	return (max - band) / (double)max;
}
	\end{minted}
	\end{minipage}
\end{listing}


\begin{listing}[ht]
	\caption{Method calculateEfficiency after manual Extract Method refactoring.}
	\label{lst:calc-eff-manual}
	\begin{minipage}{\linewidth}
		\begin{minted}[highlightlines={22,26,47,48}]{java}
private double calculateEfficiency() {
	//find the max evaluations parameter index
	int max = -1;
	int evalIndex = -1;
	int i7 = 0;
	boolean stay1 = true;
	while (stay1 && (i7 < parameterFile.size())) {
		Parameter parameter = parameterFile.get(i7);
		if (parameter.getName().equals("maxEvaluations")) {
			max = (int) parameter.getUpperBound();
			evalIndex = i7;
			stay1 = false;
		}
		if (stay1) {
			i7++;
		}
	}
	if (evalIndex == -1) {
		throw new FrameworkException("no maxEvaluations parameter");
		}
	//find lowest band reaching attainment
	int band = extracted(max, evalIndex);
	return (max - band) / (double)max;
}
	
private int extracted(int max, int evalIndex) {
	int band = max;
	int i8 = 0;
	boolean stay2 = true;
	while (stay2 && (i8 <= max - bandWidth)) {
		int count = 0;
		int total = 0;
		for (int j = 0; j < metrics.length; j++) {
			if ((parameters[j][evalIndex] >= i8) && (parameters[j][evalIndex] <= i8 + bandWidth - 1)) {
				total++;
				if (metrics[j][metric] > threshold) {
					count++;
					if (count / (double) total >= 0.9) {
						band = i8;
						stay2 = false;
					}
				}
			}
		}
		i8 += bandWidth;
	}
	return band;
}
	\end{minted}
	\end{minipage}
\end{listing}


%\begin{listing}[ht]
%	\caption{Method calculateEfficiency after manual Extract Method refactoring.}
%		\label{lst:calc-eff-manual-extract}
%		\begin{minipage}{\linewidth}
%			\begin{minted}[highlightlines={3,4,13,14,15,18,19,21,24,25}]{java}
%private int extracted(int max, int evalIndex) {
%	int band = max;
%	int i8 = 0;
%	boolean stay2 = true;
%	while (stay2 && (i8 <= max - bandWidth)) {
%		int count = 0;
%		int total = 0;
%		for (int j = 0; j < metrics.length; j++) {
%			if ((parameters[j][evalIndex] >= i8) && (parameters[j][evalIndex] <= i8 + bandWidth - 1)) {
%				total++;
%				if (metrics[j][metric] > threshold) {
%					count++;
%					if (count / (double) total >= 0.9) {
%						band = i8;
%						stay2 = false;
%					}
%				}
%			}
%		}
%		i8 += bandWidth;
%	}
%	return band;
%}
%	\end{minted}
%	\end{minipage}
%\end{listing}


